Griefing-Penalty: Countermeasure for Griefing Attack in Lightning Network

Lightning Network can execute unlimited number of off-chain payments, without incurring the cost of recording each of them in the blockchain. However, conditional payments in such networks is susceptible to Griefing Attack. In this attack, an adversary doesn't resolve the payment with the intention of blocking channel capacity of the network. We propose an efficient countermeasure for the attack, known as Griefing-Penalty. If any party in the network mounts a griefing attack, it needs to pay a penalty proportional to the collateral cost of executing a payment. The penalty is used for compensating affected parties in the network. We propose a new payment protocol HTLC-GP or Hashed Timelock Contract with Griefing-Penalty to demonstrate the utility of the countermeasure. Upon comparing our protocol with existing payment protocol Hashed Timelock Contract, we observe that the average revenue earned by the attacker decreases substantially for HTLC-GP as compared to HTLC. We also study the impact of path length for routing a transaction and rate of griefing-penalty on the budget invested by an adversary for mounting the attack. The budget needed for mounting griefing attack in HTLC-GP is 12 times more than the budget needed by attacker in HTLC, given that each payment instance being routed via path length of hop count 20.

==> security.tex <==
\subsection{Security Analysis}
\label{secgp}

\begin{theorem}
Given a payment request $(U_0,U_n,\alpha_0)$ to be transferred via path  $P=\langle U_0, U_1,\ldots,U_n \rangle$, if at least one party $U_{k}, k \in [1,n]$ mounts griefing attack then any honest party $U_j \in P, j \in [0,k-1]$ will earn compensation, without losing any funds in the process. 
\label{th11}
\end{theorem}
\textbf{Proof}:
We consider the worst-case in which we assume only a single node is honest in a path and rest of the nodes acts maliciously. We note that if fewer number of parties are corrupted, the honest nodes still interact with malicious neighbours and hence they get reduced to cases mentioned here. In particular, we analyze interactions between honest and dishonest parties in our system and ensure that honest parties do not get cheated and get their due.  

\begin{itemize}



\item \textit{\underline{Case 1 : $U_0$ is honest}} \\  In the \texttt{Pre-processing Phase}, the honest sender builds the onion packets containing terms of contract which are propagated through the nodes in the path. While the values in the packets are contingent to the values sent by R, honest S is in no position to verify it. At this point, S just follows the protocol. 

%As sender initiates the \texttt{Pre-processing Phase}, so this case can be ruled out. \todo{looks hasty. read the comment in tex file. }
% Suggested change to something like this: In the \texttt{Pre-processing Phase}, the honest sender builds the onion packets containing terms of contract which are propagated through the nodes in the path. While the values in the packets are contingent to the values sent by R, honest S is in no position to verify it. At this point, S just follows the protocol. 


In the \texttt{Two Round Locking Phase}:
\begin{itemize}
\item \emph{Establishing the Cancellation Contract}: Since $U_0$ is the last party to receive the contract, in case any party $U_i, i \in [1,n]$ griefs, then it will end up paying a cumulative penalty of $\gamma.(\Sigma_{j=1}^{i-1} (\alpha_j t_j)+(\alpha_0+\psi)t_0)$, whereby $U_0$ earns a compensation of $\gamma(\alpha_0+\psi)t_0$.



\item \emph{Establishing the Payment Contract}:  $U_0$ may not be able to forward the contract to $U_{1}$ if there is discrepancy in the terms of the outgoing contract or if $U_{1}$ has stopped responding. Since $U_n$ is dishonest, it will not release the preimage $r$ for cancelling the contracts established in the first round. As per the terms of the contract, after the elapse of locktime $t_{n-1}$, it pays a cumulative griefing-penalty $\gamma.(\Sigma_{j=1}^{n-1} (\alpha_j t_j)+(\alpha_0+\psi)t_0)$ to $U_{n-1}$. This money is used for compensating rest of the parties, starting from $U_{0}$ till $U_{n-1}$. Even if $U_1$ griefs, as per the terms of the contract it has to pay the required compensation $\gamma(\alpha_0+\psi)t_0$ to $U_0$. Hence $U_0$ will not lose funds. 
\end{itemize}

In the \texttt{Release Phase}, a similar argument can be given. Assuming that two round locking phase got executed successfully, if $U_{1}$ is not able to release the preimage corresponding to either cancellation hash or payment hash before the elapse of contract's locktime, it will have to pay a penalty to $U_0$. 





%If any other node $U_j, j \in [0,n-2]$ starts reverse-grefing as well, intentionally or due to crash fault, it will not result in loss of funds of $U_{j+1}$. This is because $U_{j+1}$ has collected the required griefing-penalty from $U_{j+2}$. 

\item \textit{\underline{Case 2 : An intermediate node $U_i, i \in [1,n-1]$ is honest}} \\ For the \texttt{Pre-processing Phase}, if $U_i$ does not receive the onion packet, the payment won't get instantiated.

In the \texttt{Two Round Locking Phase}:
\begin{itemize}[leftmargin=*]
\item \emph{Establishing the Cancellation Contract}: $U_i$ may not be able to forward the contract to $U_{i-1}$ if the latter stops responding. Since $U_n$ is dishonest, it will not release the preimage $r$ for cancelling the contracts established in the first round. As per the terms of the contract, after the elapse of locktime $t_{n-1}$, it pays a cumulative griefing-penalty $\gamma.(\Sigma_{j=1}^{n-1} (\alpha_j t_j)+(\alpha_0+\psi)t_0)$ to $U_{n-1}$. Even if $U_{i+1}$ griefs, as per the terms of the contract it has to pay the required compensation $\gamma( (\alpha_0+\psi)t_0+ \Sigma_{j=1}^{i} (\alpha_j t_j))$ to $U_i$. Since no contract has been established between $U_i$ and $U_{i-1}$, $U_i$ retains the entire compensation.

\item \emph{Establishing the Payment Contract}: $U_i$ may not be able to forward the contract to $U_{i+1}$ if  $U_{i+1}$ stops responding. The same logic stated for \emph{cancellation contract} holds true except now $U_i$ can retain $\gamma \alpha_i t_i$ as compensation and forward the rest of the amount to node $U_{i-1}$. Even if $U_{i-1}$ doesn't respond and wait for the locktime $t_{i-1}$ to elapse, $U_i$ will not lose funds.
\end{itemize}

In the \texttt{Release Phase}, $U_i$ can be griefed in the following ways:
\begin{itemize}[leftmargin=*]
\item $U_{i+1}$ withholds the preimage (either cancellation or payment) from $U_{i}$ and waits for the contract locktime to expire. In that case, $U_{i+1}$ has to pay compensation of $\gamma ((\alpha_0+\psi)t_0+ \Sigma_{j=1}^{i} (\alpha_j t_j))$ to $U_{i}$. Even if $U_{i-1}$ reverse-griefs, $U_i$ will be able to compensate without incurring any loss. 
\end{itemize}
\item  \textit{\underline{Case 3 : $U_n$ is honest}} \\ Receiver $U_n$ initiates the release of preimage. It will resolve the payment within a bounded amount of time either by releasing the preimage for payment hash or cancellation hash, as per the situation. $U_{n-1}$ cannot reverse-grief and force receiver to pay a griefing-penalty. 

\end{itemize}

%\begin{theorem}
%Given a payment request $(U_0,U_n,\alpha_0)$ to be transferred via path  $\langle U_0, U_1,\ldots,U_n \rangle$, if a party $U_j, j \in [1,n]$ griefs then it is required to pay a penalty which is used for compensating all the affected parties. Apart from the griefer, none of the honest parties lose funds in the process. 
%\label{th11}
%\end{theorem}
%\textbf{Proof Sketch}: \begin{itemize}[leftmargin=*]
%\item Receiver $U_n$ griefs: In the \texttt{Pre-processing Phase}, since $U_0$ initiates the process, $U_n$ has no role to play.
%
%In the \texttt{Two Round Locking Phase}:
%\begin{itemize}[leftmargin=*]
%\item \emph{Establishing the Cancellation Contract}: $U_n$ may not initiate the round. The payment aborts by default.
%\item \emph{Establishing the Payment Contract}: $U_n$ refuses to sign the contract forwarded by $U_{n-1}$. If it doesn't release the \emph{proof-of-cancellation} before the contract locktime expires, $U_{n-1}$ will claim the penalty $\gamma((\psi+\alpha_0)t_0 + \Sigma_{j=1}^{n-1} \alpha_{j} t_j)$, locked in the contract. 
%
%\end{itemize}
%
%In the \texttt{Release Phase}, the receiver can grief by withholding both the witnesses from $U_{n-1}$. As a consequence, it pays a cumulative penalty of $\gamma((\psi+\alpha_0)t_0 + \Sigma_{j=1}^{n-1} \alpha_{j} t_j)$. Except $U_n$, every node in the path earn the maximum compensation.
%%If any other node $U_j, j \in [0,n-2]$ starts reverse-grefing as well, intentionally or due to crash fault, it will not result in loss of funds of $U_{j+1}$. This is because $U_{j+1}$ has collected the required griefing-penalty from $U_{j+2}$. 
%
%\item Any intermediate party $U_i, i \in [1,n-1]$ griefs: For the \texttt{Pre-processing Phase}, if $U_i$ does not forward the packet, the payment won't get instantiated.
%
%In the \texttt{Two Round Locking Phase}:
%\begin{itemize}[leftmargin=*]
%\item \emph{Establishing the Cancellation Contract}: $U_i$ may either not forward the contract to $U_{i-1}$ or simply refuse to sign the contract forwarded by $U_{i+1}$. If the receiver $U_n$ is honest, then after constant amount of time it will release the preimage $r$. Hence all the reverse cancellation contracts established till $U_i$ will get settled off-chain. If $U_i$ withholds the preimage from $U_{i-1}$, it will have to pay the griefing-penalty.  
%\item \emph{Establishing the Payment Contract}: $U_i$ refuses to sign the contract forwarded by $U_{i-1}$ or doesn't forward the contract to $U_{i+1}$. The same argument will hold true. If the receiver $U_n$ is honest, then after constant amount of time it will release the preimage $r$. Hence all the reverse cancellation contracts established till $U_i$ will get settled off-chain. Only $U_i$ ends up losing money if it withholds the preimage.
%\end{itemize}
%
%In the \texttt{Release Phase}, $U_i$ can grief in the following ways:
%\begin{itemize}[leftmargin=*]
%\item It withholds the witness from $U_{i-1}$: Pays the same penalty, as it would have incurred during a griefing attack in the \texttt{Locking Phase}.
%\item If $U_i$ doesn't respond to the request off-chain termination of contract, then $U_{i+1}$ will claim its reward by revealing the preimage, either $x$ or $r$ on-chain and close the channel $(U_i,U_{i+1})$.
%\end{itemize}
%
%\item $U_0$ griefs: While executing the \texttt{Pre-processing Phase}, if the sender sends malformed packets through the path, there can be two possibilities:
%\begin{itemize}[leftmargin=*]
%\item Any intermediate parties cannot detect the error.
%\item If the packet received by the receiver doesn't confirm to the terms of the payment (insufficient locktime, wrong amount being transferred, incorrect payment hash), it will not initiate the \emph{Locking Phase.}
%\end{itemize}
%
%
%In the \texttt{Two Round Locking Phase}:
%\begin{itemize}[leftmargin=*]
%\item \emph{Establishing the Cancellation Contract}: If the sender has sent out malformed packets, an intermediate party $U_i$ can figure out the discrepancy in the contract and abort.
%
%The sender can deny accepting contract from $U_1$. If the receiver $U_n$ is honest, then after constant amount of time it will release the preimage $r$. Hence all the reverse cancellation contracts established till $U_1$ will get settled off-chain.
%
%
%\item \emph{Establishing the Payment Contract}: $U_0$ doesn't initiate the phase and goes offline. In that case, an honest receiver will wait for a constant amount of time and release the preimage $r$ in order to cancel all the contracts established in the first round.
%\end{itemize}
%
%In the \texttt{Release Phase}, $U_0$ cannot grief because it is the last node to receive a witness. Hence withhodling a solution is not an option. If $U_0$ denies accepting a witness from $U_1$, it can go on-chain and unlock its fund from the contract.
%
%
%
%\end{itemize}

%\begin{corollary}
%% If an adversary locks fund in all the channels involved in routing a self payment for a certain timeperiod, it has to bear a substantial cost for launching the attack.
%% The loss incurred disincentivizes an adversary from mounting the griefing attack by initiating a self payment. 
%If the adversary initiates a self payment and mounts a Griefing Attack, none of its objectives are fulfilled.
%\end{corollary}
%\textbf{Proof Sketch}: 

\begin{theorem}
\label{priv}
Given the information of griefing-penalty in the off-chain contract, an intermediate node cannot infer its exact position in the path for routing payment.  
\label{21}
\end{theorem}
\textbf{Proof}: For routing payment of amount $\alpha$ from $U_0$ to $U_n$ via intermediaries $U_i, i \in [1,n-1]$, several instances of off-chain contract is established across the payment channels. The amount locked by party $U_j$ and $U_{j+1}$ in their off-chain contract is $\alpha_j$ and $\gamma((\psi + \alpha_0)t_0+\Sigma_{k=1}^{k=j} \alpha_j t_{j}), j \in [0,n-1]$, respectively. Let us assume that there exists an algorithm $\tau$ which reveals the exact position of any intermediate node $D : D \in \{U_1,U_2,\ldots,U_{n-1}\}$ in the path. This implies that given the information of cumulative griefing-penalty mentioned in the contract, it can distinguish between the penalty charged by channel $(U_j,U_{j+1}), j \in [1,n-1]$ and penalty charged by channel $(U_0,U_1)$, which is $\gamma ((\psi+\alpha_0)t_0)$. However, the routing attempt cost $\psi$, was added by node $U_0$ as an extra compensation charged to cover up for routing attempt expense as well as hiding its identity from its next neighbour. This is information is private and not known by any node except $U_0$. Additionally, the value of $\psi$ is set such that $\psi t_{0} \geq  \alpha ((k+1) t_0+\Sigma_{l=1}^{k} l\Delta), k \in \mathbb{N}$. Any number being selected from $\mathbb{N}$ being equiprobable, the probability of distinguishing becomes negligible. 

Note: \emph{In practical application, there is a limit on the routing attempt fee which a sender can charge. The set from which $k$ is selected is significantly smaller compared to $\mathbb{N}$. But even under such circumstances, the best inference made by any intermediate node $U_j$ about its location is that it is located at position $(j+k)$ where $\psi t_0 > \alpha. t_0 + \alpha.(t_0+\Delta) + \alpha.(t_0+2\Delta) + \ldots + \alpha.(t_0+k\Delta), k$ acts as the blinding factor.}

